Designing an Optimal Kilonova Search using DECam for Gravitational Wave Events

We address the problem of optimally identifying all kilonovae detected via gravitational wave emission in the upcoming LIGO/Virgo/KAGRA Collaboration observing run, O4, which is expected to be sensitive to a factor of $\sim 7$ more Binary Neutron Stars alerts than previously. Electromagnetic follow-up of all but the brightest of these new events will require $>1$ meter telescopes, for which limited time is available. We present an optimized observing strategy for the Dark Energy Camera during O4. We base our study on simulations of gravitational wave events expected for O4 and wide-prior kilonova simulations. We derive the detectabilities of events for realistic observing conditions. We optimize our strategy for confirming a kilonova while minimizing telescope time. For a wide range of kilonova parameters, corresponding to a fainter kilonova compared to GW170817/AT2017gfo we find that, with this optimal strategy, the discovery probability for electromagnetic counterparts with the Dark Energy Camera is $\sim 80\%$ at the nominal binary neutron star gravitational wave detection limit for the next LVK observing run (190 Mpc), which corresponds to a $\sim 30\%$ improvement compared to the strategy adopted during the previous observing run. For more distant events ($\sim 330$ Mpc), we reach a $\sim 60\%$ probability of detection, a factor of $\sim 2$ increase. For a brighter kilonova model dominated by the blue component that reproduces the observations of GW170817/AT2017gfo, we find that we can reach $\sim 90\%$ probability of detection out to 330 Mpc, representing an increase of $\sim 20 \%$, while also reducing the total telescope time required to follow-up events by $\sim 20\%$.

==> eventsTable.tex <==
\begin{center}
\begin{table*}[H]
\begin{threeparttable}
\caption{ LVC event details. \label{tab:events}}
\hspace*{-3cm}
\begin{tabular*}{1.0\linewidth}{@{\extracolsep{\fill}}p{.05\linewidth}p{.015\linewidth}p{.03\linewidth}p{.08\linewidth}p{.04\linewidth}p{.06\linewidth}p{.06\linewidth}p{.06\linewidth}p{.06\linewidth}p{.07\linewidth}p{.085\linewidth}p{.04\linewidth}}
\toprule
Event & O\# & Type & LVC Sky Area (90\%,50\%; $\mathrm{deg}^2$)& Int. Prob. (\%) & M$_1$ ($M_\odot$) & M$_2$ ($M_\odot$) & M$_f$ ($M_\odot$) & Dist. (Mpc) & $X_{eff}$ & FAR (Yr$^{-1}$) & Network SNR\\[1ex]
\hline

170817 & 2 & BNS & 28, & 80.7?  &$1.46\substack{+0.12 \\ -0.1}$&$1.27\substack{+0.09 \\ -0.09}$& $\leq2.8$&$40\substack{+7 \\ -15}$&$0.00\substack{+0.02 \\ -0.01}$&$\leq1.0\mathrm{E}^{-07} $&33.0\\[2ex]

190510 & 3 & BNS & 91166, 31 &   65 &&&&&&& \\[2ex]

190814 & 3 & Mass gap & 19, 4 & 98&$23.2\substack{+1.1 \\ -1.0}$&$2.6\substack{+0.08 \\ -0.09}$&$25.6\substack{+1.1 \\ -0.9}$&$240\substack{+40 \\ -50}$&$0.00\substack{+0.06 \\ -0.06}$&$\leq1.0\mathrm{E}^{-05} $&22.2\\[2ex]

\hline 
\end{tabular*}
\end{threeparttable}
\end{table*}
\end{center}


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[options]{hyperref}
% To add links in your PDF file, use the package "hyperref"
% with options according to your LaTeX or PDFLaTeX drivers.
%
% ----------------
% editing macros
\newcommand\issuenord[2]{ \textbf{[}{\color{orange} ISSUE for #1} \textbf{||} \textbf{#2}\textbf{]}}
\newcommand\issuejason[2]{ \textbf{[}{\color{violet} ISSUE for #1} \textbf{||} \textbf{#2}\textbf{]}}
\newcommand\issueclecio[2]{ \textbf{[}{\color{brown} ISSUE for #1} \textbf{||} \textbf{#2}\textbf{]}}
\newcommand\changed[1]{ {\color{green}{CHANGED ||  #1}}}
\newcommand\removed[1]{ {REMOVING || \xout{#1}} }
\newcommand\responsenord[2]{ \textbf{[}{\color{orange} from #1} \textbf{||} \textbf{response: #2}\textbf{]}}
\newcommand\responsejason[2]{ \textbf{[}{\color{violet} from #1} \textbf{||} \textbf{response: #2}\textbf{]}}
\newcommand\responseclecio[2]{ \textbf{[}{\color{brown} from #1} \textbf{||} \textbf{response: #2}\textbf{]}}

\newcommand\todonow[1]{{\color{red}{TODO : #1}}}
% \newcommand\issuejason[1]{{\color{Periwinkle}{FROM JASON: #1}}}
% \newcommand\issueclecio[1]{{\color{green}{FROM CLECIO: #1}}}
% \newcommand\todolater[1]{{\color{blue}{TODO LATER: #1}}}
%\def \tb{\textcolor{blue}}


% ----------------
% commonly used phrases
\def \lenspop {{\texttt LensPop}}
\def \myfig {Fig.~}
\def \mysec {\S}
\def \myeqn {Eqn.~}
\def \mytbl {Table~}

\def \challenge {Strong Gravitational Lens Challenge}
\def \challengeabbreviation {SL Challenge}
\def \mysep {\sep} % for journal of astronomy computing
\def \mysep { -- } %  for mnras
\def \deeplensing {\emph{DeepLensing}}


% ----------------
% Science units

%\def \kms  {{\rm km\, s^{-1}}}
%\def \msol {{\rm M_{\odot}}}
%\def \sqdeg {sq. deg.\ } %{${\rm deg}^2$}
%\def \sqdegadjective {-sq.-deg.\ }
%\def \sqarcsec {{\rm arcsec}^2}
%\def \massunitshi {\times 10^{13}}
%\def \massunitslo {\times 10^{12}}
%\def \arcsec {''}

\def \thetae {\theta_{\rm E}}
\def \zsource     {z_{\rm s}}
\def \zlens       {z_{\rm l}}
\def \z           {\zlens}
\def \sigmav      {\sigma_{\rm v}}
\def \gmag {g}
\def \rmag {r}
\def \imag {i}

%-----------habib def

%\hyphenation{conhe-ci-da}

\def \dol {D_{ OL}}
\def \dos {D_{OS}}
\def \dls {D_{LS}}

\def \lt {<}

\def \dcrit {\frac{\dos}{\dol \dls}}
\def \scrit {\Sigma_{\rm crit}}
\def \dtcrit {D_{\rm ef}}
\def \vxi {\vec{\xi}}
\def \vx {\vec{x}}
\def \vy {\vec{y}}
\def \pr {\prime}
\def \dpa {\partial}
\def \g {\gamma}
\def \k {\kappa}
\def \al {\alpha}
\def \l {\lambda}
\def \val {\vec{\al}}
\def \vp {\varphi}
\def \va {\varphi}
\def \sen {\textrm{\,sen}\,}
\def \eps {\varepsilon}
\def \zxi {(\dol\xi/r_s)}
\def \arcth {{\rm arctanh}}
\def \kse{\kappa^{\varphi}_{s}}
\def \ksel{\kappa^{\Sigma}_{s}}
\def \ke{\kappa_{\varepsilon}}
\def \ksiep{\kappa_{\rm SIEP}}
\def \kpnfw{\kappa_{\rm PNFW}}
\def \ksie{\kappa_{\rm SIEP}}
\def \kenfw{\kappa_{\rm PNFW}}
\def \es {\varepsilon_\Sigma}
%\def \xe {\tilde{x}}
%\def \xe {x_\eps}
%\def \pe {\phi_\eps}
%
\def \xe {\tilde{x}}
\def \pe {\tilde{\phi}}
%
%\def \bphi{\tilde{\phi}}
%\def \bs{\tilde{S}}
%\def \bsi{\tilde{s}}
%
\def \bphi{\bar{\phi}}
\def \bs{\bar{S}}
\def \bsi{\bar{s}}
%
%
\def \hxe {\hat{\tilde{x}}}
\def \hpe {\hat{\tilde{\phi}}}

\def \beq {\begin{equation}}
\def \eeq {\end{equation}}
\def \beqn {\begin{equation*}}
\def \eeqn {\end{equation*}}



\newcommand{\f}{\text{fid}}

\newcommand{\Unif}{\ensuremath{\mathcal{U}}}



%%% Journal names
\def\ieeesc{IEEE Trans.\ Appl.\ Supercon.}
\def\sovast{Sov.\ Ast.}
\def\aap{Astr. \& Astroph.}
\def\aaps{Astr. \& Astroph., Supp.}
\def\ap{Appl.\  Phys.}
\def\apl{Appl.\ Phys.\ Lett.}
\def\aj{Astron.\ J.}
\def\pasp{Pub.\ of\ the\ Astron.\ Soc.\ of\ the\ Pacific.}
\def\apj{Astrophys.\ J.}
\def\apjl{Astrophys.\ J.\ Lett.}
\def\apjs{Astrophys.\ J.\ Suppl.}
\def\astropart{Astropart.\ Phys.}
\def\baas{Bull. Am. Astron. Soc.}
\def\jap{J.\ Appl.\  Phys.}
\def\jetplett{JETP\ Lett.}
\def\nat{Nature}
\def\mnras{Mon.\ Not.\ Roy.\ Astron.\ Soc.}
\def\nima{Nucl.\ Instrum.\ Methods\ Phys.\ Res.,\ Sect.\ A}
\def\newastr{New\ Astron.}
\def\newastrev{New\ Astron.\ Rev.}
\def\nucphysb{Nucl.\ Phys.\ B}
\def\nucphysbsupp{Nucl.\ Phys.\ B\ Proc. Supp.}
\def\nuovocim{Il\ Nuovo\ Cim.}
\def\pl{Phys.\ Lett.}
\def\plb{Phys.\ Lett.\ B}
\def\physrep{Phys.\ Rep.}
\def\physscripta{Phys.\ Scr.}
\def\pra{Phys.\ Rev.\ A}
\def\prb{Phys.\ Rev.\ B}
\def\prc{Phys.\ Rev.\ C}
\def\prd{Phys.\ Rev.\ D}
\def\pre{Phys.\ Rev.\ E}
\def\prl{Phys.\ Rev.\ Lett.}
\def\prthphys{Prog.\ Theor.\ Phys.}
\def\pspie{Proc.\ Soc.\ Photo-Opt.\ Instrum.\ Eng.}
\def\rmp{Rev.\ Mod.\ Phys.}
\def\rsi{Rev.\ Sci.\ Instr.}
\def\sci{Science}
\def\jcap{JCAP\ }

==> packages.tex <==

% \usepackage{subfigure}
%\usepackage{color}
\usepackage{threeparttable}
\usepackage{multirow}
%\usepackage{hyperref}
\usepackage{lineno}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{pdflscape}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{caption}
\usepackage{subcaption}
\captionsetup{compatibility=false}
%\usepackage{bm}		% Bold maths symbols, including upright Greek

\usepackage{url}
%\usepackage{mathptmx}
%\usepackage{txfonts}
%\usepackage{ae}
%\usepackage{aecompl}
\usepackage{amsmath}	% Advanced maths commands
%\usepackage{amssymb}	% Extra maths symbols
%\usepackage[hidelinks]{hyperref}       % hyperlinks
\usepackage{txfonts}
\usepackage{setspace}
\usepackage[normalem]{ulem}


==> tb_app.tex <==
\begin{longtable*}{cllllll}
%\small
\caption{\label{tab:app}  Strategy Detection Probabilities in diferent sky conditions for red and blue Kilonovas on the three events that were follow-up during O2 and O3 with DECAM. }\\
%\begin{tabular}
\hline \hline
Event &  Strategy & Component & Sky  &  Detection Probability & Telescope time  \\


 \endfirsthead

 \hline
 \multicolumn{7}{|c|}{Continuation of Table }\\
 \hline
Event &  Strategy & Component & Sky  &  Detection Probability & Telescope time  \\
 \hline
 \endhead

 \hline
 \endfoot




\hline \hline 

GW170817 &  Top  &  red   &  moony & prob & time   \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& LowTT   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
\hline
& ED   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& LD   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& O3   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
 \hline

GW190814 &  Top  &  red   &  moony & prob & time   \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& LowTT   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
\hline
& ED   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& LD   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& O3   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
  \hline
 \hline
GW170817 &  Top  &  red   &  moony & prob & time   \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& LowTT   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
  \hline
& ED   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& LD   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\
 \hline
& O3   &    red  &   moony & prob & time \\
 &    &     &  not moony & prob & time \\
 &    &  blue   &   moony & prob & time \\
 &    &      &  not moony & prob & time \\



\hline \hline
%\end{tabular}
\\
\end{longtable*}

==> tb_o3sumarize.tex <==
%old_strategy=[90.0,200.0,'zi',0.25,1.0,0.9]
\begin{table}
\small
\caption{\label{tab:sample_description} Reference Observational Strategies inspired in previous DECam searches. As the strategies were not homogeneous, we select some typical parameters to construe a reference strategy for the sake of comparison to the optimized ones. These numbers does not represent a specific follow-up event. \nfs{Suggested Removal}}

\begin{tabular}{lllllll}
%\hline\hline
%Exposure time 1 & filter 1 & Time of Obs 1 & Exposure time 2 & filter 2 & Time of Obs 2 & Sky area prob coverage   \\

\hline \hline 
First Night (0.5 days)\\

\hline
Exposure time  &$90$ & \\
Filter & $i$ & $z$ \\
\hline \hline
Second Night (1.5 day)\\
\hline 
Exposure time  & $90$ &\\
Filter  & $i$ & $z$ \\

Sky area prob coverage & $90\%$ & $90\%$  \\


\hline \hline
\end{tabular}
\end{table}

